Exponential Family Model-Based Reinforcement Learning via Score Matching

We propose an optimistic model-based algorithm, dubbed SMRL, for finite-horizon episodic reinforcement learning (RL) when the transition model is specified by exponential family distributions with $d$ parameters and the reward is bounded and known. SMRL uses score matching, an unnormalized density estimation technique that enables efficient estimation of the model parameter by ridge regression. Under standard regularity assumptions, SMRL achieves $\tilde O(d\sqrt{H^3T})$ online regret, where $H$ is the length of each episode and $T$ is the total number of interactions (ignoring polynomial dependence on structural scale parameters).

==> acknowledgements.tex <==
\section*{Acknowledgements}
We thank Pritish Kamath, Danica J. Sutherland, Akshay Krishnamurthy, and Wen Sun for helpful discussions. Part of this work was done while GL, ZW, and ZY were participating in the Simons Program on the Theoretical Foundations of Reinforcement Learning in Fall 2020. Part of this work was done while JL was interning with ZW from August 2020 to February 2021.
